PAg-NeRF: Towards fast and efficient end-to-end panoptic 3D representations for agricultural robotics

Precise scene understanding is key for most robot monitoring and intervention tasks in agriculture. In this work we present PAg-NeRF which is a novel NeRF-based system that enables 3D panoptic scene understanding. Our representation is trained using an image sequence with noisy robot odometry poses and automatic panoptic predictions with inconsistent IDs between frames. Despite this noisy input, our system is able to output scene geometry, photo-realistic renders and 3D consistent panoptic representations with consistent instance IDs. We evaluate this novel system in a very challenging horticultural scenario and in doing so demonstrate an end-to-end trainable system that can make use of noisy robot poses rather than precise poses that have to be pre-calculated. Compared to a baseline approach the peak signal to noise ratio is improved from 21.34dB to 23.37dB while the panoptic quality improves from 56.65% to 70.08%. Furthermore, our approach is faster and can be tuned to improve inference time by more than a factor of 2 while being memory efficient with approximately 12 times fewer parameters.

==> contribs/datasets.tex <==
\section{Datset}
\label{sec:datasets}

We evaluate our models in a very challenging agricultural datasets Horticulture Glasshouse Sweet Pepper (BUP20)~\cite{smitt2021}.
It consists of RGB-D images captured with off-the-shelf sensors captured by the autonomous phenotyping platform PATHoBot driving at $0.2 m/s$ at a glasshouse environment in Campus Kleinaltendorf (CKA) of the university of Bonn.
Moreover, the dataset present high detail panoptic segmentation, labels alongside panoptic predictions from an instance segmentation model pre-trained on these domains.
~
\begin{figure}[!t]
    \vspace{12pt}
    \centering
    \includegraphics[width=\linewidth]{figures/dataset.png}
    \caption{Datasets example placeholder}
    \label{fig:dbexample}
    \vspace{-16pt}
    % \vspace{-16pt}
\end{figure}
~
A collection of 10 sequences are included, with two sweet pepper cultivar \textit{Mavera} (yellow) and \textit{Allrounder} (red). Both Cultivars matured from green, to mixed, to their primary color. 
The dataset includes RGB-D images captured also with an Intel RealSense D435i, as well as IMU data and wheel odometry.
In this case we evaluate our models on a panoptic segmentation task with only 2 semantic classes (fruit and background).

The dataset has sparse non-overlapping instance based segmentation annotations, and we generate short sequences around them for validation and training of N and M frames long.
Alongside the sparse-labels, for all frames we pre-compute panoptic detections using a pre-trained Panoptic DeepLab model from prior work~\cite{crop_agnostic_halstead2021crop}, in order to train our model's panoptic heads.

Tab.~\ref{tab:datasets} summarizes the attributes of the dataset.

% , for both SB20 and BUP20 datasets, and Fig.\ref{fig:datasets} shows some typical image samples.
\begin{table}[!b]
    \vspace{-5mm}
	\centering
	\caption{BUP20 dataset characteristics}
	\begin{tabular}{ccc cc}
        Image Size & fps & Train & Val. & Eval.\\\hline
     $1280\times720$ & 15 & 124 & 62 & 93 \\
    \end{tabular}
	\label{tab:datasets}
\end{table}


